On the impact of observation error correlations in data assimilation, with application to along-track altimeter data

Data assimilation involves estimating the state of a system by combining observations from various sources with a background estimate of the state. The weights given to the observations and background state depend on their specified error covariance matrices. Observation errors are often assumed to be uncorrelated even though this assumption is inaccurate for many modern data-sets such as those from satellite observing systems. As methods allowing for a more realistic representation of observation-error correlations are emerging, our aim in this article is to provide insight on their expected impact in data assimilation. First, we use a simple idealised system to analyse the effect of observation-error correlations on the spectral characteristics of the solution. Next, we assess the relevance of these results in a more realistic setting in which simulated alongtrack (nadir) altimeter observations with correlated errors are assimilated in a global ocean model using a three-dimensional variational assimilation (3D-Var) method. Correlated observation errors are modelled in the 3D-Var system using a diffusion operator. When the correlation length scale of observation error is small compared to that of background error, inflating the observation-error variances can mitigate most of the negative effects from neglecting the observation-error correlations. Accounting for observation-error correlations in this situation still outperforms variance inflation since it allows small-scale information in the observations to be more effectively extracted and does not affect the convergence of the minimization. Conversely, when the correlation length scale of observation error is large compared to that of background error, the effect of observation-error correlations cannot be properly approximated with variance inflation. However, the correlation model needs to be constructed carefully to ensure the minimization problem is adequately conditioned so that a robust solution can be obtained. Practical ways to achieve this are discussed.

==> app_normalization.tex <==

While only \eq{\bR^{-1}} is required `online' (\textit{i.e.}, at each iteration of the minimization), \eq{\bR} or its square root are required `offline' during the initialization of the assimilation cycle to estimate the normalization factors in \eq{\bGamma}. In order to apply either \eq{\bD} or its square root, linear systems solutions are required. Exploiting the fact that \eq{\bM} is diagonal with mass lumping, we first reformulate \eq{\bD} as:
\begin{equation}
   \bD = \bM^{1/2} \left[\left(\bI + \bM^{-1/2}\bA\bM^{-1/2}\right)^{-1} \right]^{m/2} \left[\left(\left(\bI + \bM^{-1/2}\bA\bM^{-1/2}\right)^{- 1}\right)^{\rm T} \right]^{m/2} \bM^{1/2},
   \label{eq_inv_D_alt}
\end{equation}

To solve the system defined by \eq{\bI + \bM^{-1/2}\bA\bM^{-1/2}}, a Chebyshev Iteration (CI) algorithm has been implemented following \citet{Weaver_2016}. The use of a transpose on the inverse of \eq{\bI + \bM^{-1/2}\bA\bM^{-1/2}} even though it is symmetrical is important because, in practice, the CI algorithm is truncated before its full convergence. The adjoint of the CI algorithm is thus used for half of the system solutions so that the symmetry of \eq{\bD} is preserved by construction even in the presence of substantial truncation error.\par

The CI algorithm requires \textit{a priori} lower and upper bounds of the extremal eigenvalues of \eq{\bI + \bM^{-1/2}\bA\bM^{-1/2}}: the more accurate the bounds, the faster the convergence. Following \citet{Weaver_2016}, we chose to estimate these extremal eigenvalues with a Conjugate Gradient (CG) algorithm. Note that we attempted to use an analytical upper bound based on Theorem 3.1 of \citet{Loghin_2006} (and a lower bound set to 1) to replace the CG algorithm, but chose not to use it in the end: this upper bound is pessimistic, while running once the CG/Lanczos to obtain accurate estimates and a faster convergence of the CI does not add any substantial cost compared to the rest of the initialization of the assimilation cycle. Still following \citet{Weaver_2016}, the CI algorithm is run once at initialization to estimate the number of iteration required to reach the target tolerance of the residual norm. Then, the CI algorithm is systematically run for this fixed number of iterations both in the direct and adjoint solvers (CFI algorithm in \citet{Weaver_2016}), removing the need for estimation of the norm of the residual and avoiding any communication between different processors outside of the halo exchange realised before applying \eq{\bI + \bM^{-1/2}\bA\bM^{-1/2}}.

A few methods have been developed to estimate normalization factors in \eq{\bB} \citep{Weaver_2021} and could also be applied in \eq{\bR}. One of them is the "brute-force" method: apply a diffusion operator to a vector equal to 0 everywhere but at the \eq{i}-th observation location. The amplitude of the output of the diffusion operator at the \eq{i}-th location is the square of the inverse of the \eq{i}-th normalization factor. Repeating this procedure for every observation location would give a complete estimation of the normalization factors. Though this approach is not the most efficient in the context of background error correlations modelling, it can be improved for nadir altimeter data. \par
Points separated by a distance large compared to the correlation length scale of the operator do not interact significantly through diffusion. Consequently, and as the operator is linear, we can thus estimate multiple normalization factors with a single call to a diffusion operator by using as an input a vector equal to 1 in regularly space locations separated by at least \eq{r} times the correlation length scale instead of in a single lcoation. If \eq{r} is too small, normalization factors will be overestimated due to their interactions through diffusion. If \eq{r} is increased, the number of normalization factor estimated per call to the diffusion operator will decrease until the method become similar the `traditional' brute-force method. In the case of nadir altimeters, empirical results seem to indicate that a value of \eq{r=5} is sufficient to obtain an average relative error of \eq{10^{-4}}, which is an order of magnitude smaller than the error obtained with the method used operationally for \eq{\bB} (randomization method with 10000 samples). With an observation error correlation length scale of 125 kilometres, \eq{r=5}, and altimeter observations separated by 20 km on average, this method requires only about 32 calls to a diffusion operator (instead of 100000 with the operational method of choice for \eq{\bB}) to evaluate the normalization factors. However, this method does not necessarily scale well in 2D or 3D.

